Just SLaQ When You Approximate: Accurate Spectral Distances for Web-Scale Graphs

Graph comparison is a fundamental operation in data mining and information retrieval. Due to the combinatorial nature of graphs, it is hard to balance the expressiveness of the similarity measure and its scalability. Spectral analysis provides quintessential tools for studying the multi-scale structure of graphs and is a well-suited foundation for reasoning about differences between graphs. However, computing full spectrum of large graphs is computationally prohibitive; thus, spectral graph comparison methods often rely on rough approximation techniques with weak error guarantees. In this work, we propose SLaQ, an efficient and effective approximation technique for computing spectral distances between graphs with billions of nodes and edges. We derive the corresponding error bounds and demonstrate that accurate computation is possible in time linear in the number of graph edges. In a thorough experimental evaluation, we show that SLaQ outperforms existing methods, oftentimes by several orders of magnitude in approximation accuracy, and maintains comparable performance, allowing to compare million-scale graphs in a matter of minutes on a single machine.

==> data/param-sensitivity-m.tex <==
m	 error
2	 0.02170
5	 0.00617
10	 0.00067
20	 0.00032
50	 0.00027
100	 0.00027

==> data/param-sensitivity-nv.tex <==
nv	 error
2   0.00184
5   0.00127
10	 0.00106
50	 0.00077
100	 0.00070
200	 0.00066
500	 0.00064
1000	 0.00065
2000	 0.00063
5000	 0.00063
